A Simpler Alternative: Minimizing Transition Systems Modulo Alternating Simulation Equivalence

This paper studies the reduction (abstraction) of finite-state transition systems for control synthesis problems. We revisit the notion of alternating simulation equivalence (ASE), a more relaxed condition than alternating bisimulations, to relate systems and their abstractions. As with alternating bisimulations, ASE preserves the property that the existence of a controller for the abstraction is necessary and sufficient for a controller to exist for the original system. Moreover, being a less stringent condition, ASE can reduce systems further to produce smaller abstractions. We provide an algorithm that produces minimal AS equivalent abstractions. The theoretical results are then applied to obtain (un)schedulability certificates of periodic event-triggered control systems sharing a communication channel. A numerical example illustrates the results.

==> Figures/S1.tex <==
\begin{figure}
    \centering
    \footnotesize
    \begin{tikzpicture} [node distance = 1.75cm, on grid, auto]
        \node (q00) [state with output, initial] {$q_{0,1}$ \nodepart{lower} \texttt{T}};
        \node (q01) [state with output, right = of q00] {
            $q_{0,2}$ \nodepart{lower} \texttt{W}    };
        \node (q10) [state with output, initial, below = of q00] {$q_{1,1}$ \nodepart{lower} \texttt{T}};
        \node (q11) [state with output, right = of q10] {
            $q_{1,2}$ \nodepart{lower} \texttt{W}};
        \node (q12) [state with output, right = of q11] {
            $Q$ \nodepart{lower} \texttt{W}};
            
        \path [-stealth, thick]
            (q00) edge node {\texttt{w}}   (q01)
            (q00) edge [loop above]  node {\texttt{s}} (q00)
            (q01) edge [bend right] node[above] {\texttt{w, s}}   (q00)
            (q01) edge node {\texttt{w, s}}   (q10)
            (q10) edge node {\texttt{w}}   (q11)
            (q10) edge [loop above]  node {\texttt{s}} (q10)
            (q11) edge [bend left] node[above] {\texttt{s}}   (q10)
            (q11) edge node {\texttt{w}}   (q12)
            (q12) edge [bend left] node {\texttt{w, s}}   (q10);
    \end{tikzpicture}
    \caption{System of Fig.~\ref{fig:twexample} after step 1, where $Q = \{(q_{1,3}), (q_{1,4})\}$.}
    \label{fig:S1}
\end{figure}
